Higher operations in string topology of classifying spaces

Examples of non-trivial higher string topology operations have been regrettably rare in the literature. In this paper, working in the context of string topology of classifying spaces, we provide explicit calculations of a wealth of non-trivial higher string topology operations associated to a number of different Lie groups. As an application of these calculations, we obtain an abundance of interesting homology classes in the twisted homology groups of automorphism groups of free groups, the ordinary homology groups of holomorphs of free groups, and the ordinary homology groups of affine groups over the integers and the field of two elements.

==> declarations.tex <==
\usepackage{amsfonts, amssymb, amsmath, eucal, amsthm, stmaryrd, verbatim}
\usepackage[all,cmtip]{xy}
%\xyoption{ps}
%\xyoption{dvips}
\usepackage{mathtools}

\makeatletter

% Formatting
%\usepackage{mathptmx}
\DeclareSymbolFont{cmlargesymbols}{OMX}{cmex}{m}{n}
%\usepackage[vmargin=3.2cm, hmargin=3.4cm]{geometry}
%\usepackage[vmargin=3.2cm, hmargin=3.4cm]{geometry}
\usepackage[vmargin=3.2cm]{geometry}
%\parindent=12pt
%\parskip=6pt plus3pt minus3pt

\usepackage{color}
\usepackage{hyperref}  
\hypersetup{%
  bookmarksnumbered=true,%
%  bookmarks=true,%
  colorlinks=true,%
  linkcolor=blue,%
  citecolor=blue,%
  filecolor=blue,%
  menucolor=blue,%
%  pagecolor=blue,%
  urlcolor=blue,%
  pdfnewwindow=true,%
  pdfstartview=}
%\usepackage{txfonts}


%\usepackage[notref,notcite]{showkeys}
\usepackage{threeparttable}
%\usepackage{booktabs}


% marginal notes e.g. \mnote{blah blah}
\newcommand\mnote[1]{\marginpar{\tiny #1}}
\setlength{\marginparsep}{0.2cm}
\setlength{\marginparwidth}{2.5cm}
\setlength{\marginparpush}{0.5cm}

\newcommand{\acomment}[1]{\footnote{#1}}

%%% Environment Definitions:

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{conjecture}[lemma]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{note}[lemma]{Note}
\newtheorem{example}[lemma]{Example}
\newtheorem{examples}[lemma]{Examples}
\newtheorem{remark}[lemma]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{question}[lemma]{Question}
\newtheorem*{acknowledgments}{Acknowledgments}
\newtheorem{notation}[lemma]{Notation}
\newtheorem{construction}[lemma]{Construction}
\numberwithin{lemma}{section}

\newtheorem{step}{Step}

%%% Symbol Commands:

\newcommand{\g}{\mathfrak{g}}
\newcommand{\Diff}{\mathrm{Diff}}
\newcommand{\Homeo}{\mathrm{Homeo}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\pt}{\mathrm{pt}}
\newcommand{\free}{\mathrm{free}}
\newcommand{\OC}{{\mathcal{OC}}}
\newcommand{\Vect}{\mathrm{Vect}}
\newcommand{\Fun}{\mathrm{Fun}}
\newcommand{\fun}{\mathrm{fun}}
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\Map}{\mathrm{Map}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\Cyl}{\mathrm{Cyl}}
\newcommand{\vertical}{\mathrm{vert}}
\newcommand{\hAut}{\mathrm{hAut}}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\Hol}{\mathrm{Hol}}
\newcommand{\Aff}{\mathrm{Aff}}

\newcommand{\bp}{\mathrm{bp}}
\newcommand{\hg}{\mathrm{hg}}
\newcommand{\ds}{\mathrm{ds}}
\newcommand{\mfld}{\mathrm{man}}

\DeclareMathOperator{\Ob}{Ob}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\Sing}{Sing}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Tot}{Tot}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

\newcommand{\N}{\mathbf{N}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\T}{\mathbb{T}}

\newcommand{\modmod}{{\slash\!\!\slash}} % Like \sslash, but with better spacing.
\renewcommand{\sslash}{\modmod}

% The category of families of h-graphs with basepoints.
\newcommand{\calHbp}{\widetilde\calH}

% External operations on families of cobordisms
\newcommand{\ucirc}{\mathbin{\underline{\circ}}}
\newcommand{\usqcup}{\mathbin{\underline{\sqcup}}}

% Notation for the forgetful and inclusion functors
\newcommand{\forget}{\mathrm{forget}}
\newcommand{\inclusion}{\mathrm{incl}}

%%% Arrows

% Slashed arrows, based on Andrew Stacey's code at
%
% http://tex.stackexchange.com/questions/13938/how-do-i-create-the-negated-arrow-on-xrightarrow
%
% and Shulman's decls.tex.
\def\slashedarrowfill@#1#2#3#4#5{%
  $\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
   \relax#5#1\mkern-7mu%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mathclap{#3}\mathclap{#2}%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mkern-7mu#4$%
}
\def\rightslashedarrowfill@{%
  \slashedarrowfill@\relbar\relbar\mapstochar\rightarrow}
\newcommand\xhto[2][]{%
  \ext@arrow 1579{\rightslashedarrowfill@}{#1}{#2}}

\newcommand{\hto}{\xhto{}}

% Replacement for xrightarrow, with shorter name and 
% the same spacing as the slashed arrow above.
\newcommand\xto[2][]{%
  \ext@arrow 1579{\rightarrowfill@}{#1}{#2}}

\newcommand\xot[2][]{%
  \ext@arrow 5197{\leftarrowfill@}{#1}{#2}}
  
  
\providecommand*{\twoheadrightarrowfill@}{%
  \arrowfill@\relbar\relbar\twoheadrightarrow
}

\newcommand\xtwoheadrightarrow[2][]{%
  \ext@arrow 1579\twoheadrightarrowfill@{#1}{#2}%
}

% Long versions
\newcommand{\longhto}{\xhto{\quad}}
\newcommand{\longto}{\xto{\quad}}
\newcommand{\longot}{\xot{\quad}}

\newcommand{\longincl}{\xhookrightarrow{\quad}}
\newcommand{\longrevincl}{\xhookleftarrow{\quad}}
\newcommand{\longtwoheadto}{\xtwoheadrightarrow{\quad}}



%%% Misc commmands

\newcommand{\tensor}{\otimes}
\newcommand{\smashprod}{\wedge}

\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\mathrm{Id}}

\newcommand{\isom}{\approx}
\newcommand{\homot}{\simeq}
\newcommand{\nhomot}{\not\simeq}
\newcommand{\homeom}{\approx}

\newcommand{\suspension}{\Sigma}
\newcommand{\loops}{\Omega}

\newcommand{\bdry}{\partial}

%\newcommand{\ho}{\mathrm{Ho}\,} % Notation for homotopy category
\DeclareMathOperator{\ho}{Ho} % Notation for homotopy category

\newcommand{\invlim}{\varprojlim}
\newcommand{\dirlim}{\varinjlim}

\newcommand{\incl}{\hookrightarrow}
\newcommand{\goesto}{\xrightarrow}
\newcommand{\cl}[1]{\overline{#1}} %closure

\DeclareMathOperator{\colim}{colim}
\newcommand{\im}{\mathrm{Im}\,}
\providecommand{\ker}{}
\renewcommand{\ker}{\mathrm{Ker}\,}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\diam}{diam}

\newcommand{\ev}{\mathrm{ev}}
\newcommand{\pr}{\mathrm{pr}}
\newcommand{\foldmap}{\nabla}



% Notation for our double categories

\newcommand{\cob}{\mathbb{C}\mathbf{ob}}
\newcommand{\cobbp}{\cob^{\mathrm{bp}}}
\newcommand{\gpd}{\mathbb{G}}
\newcommand{\man}{\mathbb{M}}
\newcommand{\pmor}{\mathbb{P}\mathbf{Mor}}

% Notation for 2-categories

\newcommand{\Cat}{\mathcal{C}\mathit{at}} % 2-cat of categories
\newcommand{\Dbl}{\mathcal{D}\mathit{bl}} % 2-cat of double categories
\newcommand{\Fib}{\mathcal{F}\mathit{ib}} % 2-cat of fibrations

% Opposites
\newcommand{\co}{\mathrm{co}} % reverse 2-morphisms
\newcommand{\op}{\mathrm{op}}
\newcommand{\hop}{\mathrm{hop}}
\newcommand{\fop}{\mathrm{fop}}



%%% Blackboard bold letters

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%%% Calligraphic letters

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

%%% Fraktur letters

\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}

\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fb}{\mathfrak{b}}
\newcommand{\fc}{\mathfrak{c}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fe}{\mathfrak{e}}
\newcommand{\ff}{\mathfrak{f}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fh}{\mathfrak{h}}
%\newcommand{\fi}{\mathfrak{i}} % already defined!
\newcommand{\fj}{\mathfrak{j}}
\newcommand{\fk}{\mathfrak{k}}
\newcommand{\fl}{\mathfrak{l}}
\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fo}{\mathfrak{o}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fr}{\mathfrak{r}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\ft}{\mathfrak{t}}
\newcommand{\fu}{\mathfrak{u}}
\newcommand{\fv}{\mathfrak{v}}
\newcommand{\fw}{\mathfrak{w}}
\newcommand{\fx}{\mathfrak{x}}
\newcommand{\fy}{\mathfrak{y}}
\newcommand{\fz}{\mathfrak{z}}

%%% Sans Serif letters

\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}

\makeatother




%Tikz 
\usepackage{tikz}
\usetikzlibrary{decorations.markings,decorations.pathreplacing,arrows}
\tikzset{
->-/.style={decoration={markings, mark=at position .5 with {\arrow{>}}},postaction={decorate}},
-<-/.style={decoration={markings, mark=at position .5 with {\arrow{<}}},postaction={decorate}},
ARC/.style ={draw=black,line join=miter,line cap=butt,miter limit=4.00,line width=0.5 mm},
TEXTARC/.style ={draw=black,line join=miter,line cap=butt,miter limit=4.00,line width=0.3 mm},
REGION/.style={draw=none, fill=white!#1!black},
REGION/.default = 80,
}
%\tikzexternalize
%\tikzsetexternalprefix{figures/}


% Ticks and crosses
\newcommand{\tickYes}{\checkmark}
\usepackage{pifont}
\newcommand{\tickNo}{\hspace{1pt}\ding{55}}


